GMT: Enhancing Generalizable Neural Rendering via Geometry-Driven Multi-Reference Texture Transfer

Novel view synthesis (NVS) aims to generate images at arbitrary viewpoints using multi-view images, and recent insights from neural radiance fields (NeRF) have contributed to remarkable improvements. Recently, studies on generalizable NeRF (G-NeRF) have addressed the challenge of per-scene optimization in NeRFs. The construction of radiance fields on-the-fly in G-NeRF simplifies the NVS process, making it well-suited for real-world applications. Meanwhile, G-NeRF still struggles in representing fine details for a specific scene due to the absence of per-scene optimization, even with texture-rich multi-view source inputs. As a remedy, we propose a Geometry-driven Multi-reference Texture transfer network (GMT) available as a plug-and-play module designed for G-NeRF. Specifically, we propose ray-imposed deformable convolution (RayDCN), which aligns input and reference features reflecting scene geometry. Additionally, the proposed texture preserving transformer (TP-Former) aggregates multi-view source features while preserving texture information. Consequently, our module enables direct interaction between adjacent pixels during the image enhancement process, which is deficient in G-NeRF models with an independent rendering process per pixel. This addresses constraints that hinder the ability to capture high-frequency details. Experiments show that our plug-and-play module consistently improves G-NeRF models on various benchmark datasets.

==> tables_main_camera_ready/r1.tex <==
\begin{table}[t]
\centering
\Huge
\caption{Comparison according to two reference views.}
% \vspace{-10pt}
\resizebox{0.95\textwidth}{!}{%
\setlength{\tabcolsep}{10pt}
\begin{tabular}{c||c|c|c||c|c|c||c|c|c}
\hline
\multirow{2}{*}{Model} &  \multicolumn{3}{c||}{\cellcolor[HTML]{C5C5C5}DTU} &  \multicolumn{3}{c||}{\cellcolor[HTML]{C5C5C5}Synthetic NeRF} &  \multicolumn{3}{c}{\cellcolor[HTML]{C5C5C5}Real Forward-Facing}     \\
\cline{2-10}
           & PSNR($\uparrow$)    & SSIM($\uparrow$)    & LPIPS($\downarrow$) & PSNR($\uparrow$)    & SSIM($\uparrow$)    & LPIPS($\downarrow$) & PSNR($\uparrow$)    & SSIM($\uparrow$)    & LPIPS($\downarrow$)  \\
\hline
NeRFLiX  & 28.54	&0.906	&0.103	&28.79	&0.926&	0.062	&25.65	&\textbf{0.844}&	0.143 \\
\hline
Ours    &\textbf{28.63}	&\textbf{0.919}	&\textbf{0.091}&	\textbf{28.85}	&\textbf{0.934}	&\textbf{0.057}	&\textbf{25.66}&	0.843	&\textbf{0.133}   \\
% \hline
\Xhline{3\arrayrulewidth}
\end{tabular}
}
\label{table:rebuttal_ref2}
% \vspace{-28pt}
\end{table}

==> tables_main_camera_ready/r2.tex <==
\begin{table}[t]
\centering
\Huge
% \vspace{5pt}
\caption{Results on per-scene optimization NeRFs.}
% \vspace{-10pt}
\resizebox{0.7\textwidth}{!}{%
\setlength{\tabcolsep}{10pt}
\begin{tabular}{c||c|c|c||c|c|c}
% \hline
\Xhline{3\arrayrulewidth}
\multirow{2}{*}{Model} &  \multicolumn{3}{c||}{\cellcolor[HTML]{C5C5C5}DVGO~\cite{sun2022direct}} &  \multicolumn{3}{c}{\cellcolor[HTML]{C5C5C5}TensoRF~\cite{chen2022tensorf}}     \\
\cline{2-7}
           & PSNR($\uparrow$)    & SSIM($\uparrow$)    & LPIPS($\downarrow$) & PSNR($\uparrow$)    & SSIM($\uparrow$)    & LPIPS($\downarrow$) \\
% \hline
\Xhline{3\arrayrulewidth}
w/o Ours  & 26.56	&0.847	&0.165	&25.97	&0.830&	0.177 \\
\hline
Ours      & \textbf{26.82}	& \textbf{0.863}	&\textbf{0.144}	&\textbf{26.23}	&\textbf{0.848}&	\textbf{0.153}  \\
% \hline
\Xhline{3\arrayrulewidth}
\end{tabular}
}
\label{table:rebuttal_dvgo}
% \vspace{-18pt}
\end{table}
